Toward the Cure of Privacy Policy Reading Phobia: Automated Generation of Privacy Nutrition Labels From Privacy Policies

Software applications have become an omnipresent part of modern society. The consequent privacy policies of these applications play a significant role in informing customers how their personal information is collected, stored, and used. However, customers rarely read and often fail to understand privacy policies because of the ``Privacy Policy Reading Phobia'' (PPRP). To tackle this emerging challenge, we propose the first framework that can automatically generate privacy nutrition labels from privacy policies. Based on our ground truth applications about the Data Safety Report from the Google Play app store, our framework achieves a 0.75 F1-score on generating first-party data collection practices and an average of 0.93 F1-score on general security practices. We also analyse the inconsistencies between ground truth and curated privacy nutrition labels on the market, and our framework can detect 90.1% under-claim issues. Our framework demonstrates decent generalizability across different privacy nutrition label formats, such as Google's Data Safety Report and Apple's App Privacy Details.

==> 11_script.tex <==
% How to select apps

\cite{geodiff}: top 200 apps in each of our 22 categories
\cite{PETS_2019}:
We annotated the policies linked from the Play Store pages of all apps
with more than 50 million installs (n = 247). In addition, we annotated the policies of randomly selected apps with more than 5 million installs (n = 103).
\cite{GDPR_ARTICLE13}: we aim at
collecting a set of high quality privacy policies with diverse application
categories.

(1) the privacy policies of applications which are in the top list of Google Play; and (2) the privacy policies should be from diverse categories since different categories may have different requirements on accessing user information. The privacy policies we collect cover 22 application categories, such as Communication, Game, and Business.

Note that there may be some noise in the crawled privacy policies. To ensure the quality of the collected privacy policy documents, we filter the crawled privacy policies with the following criteria: (1) the privacy policy is written in English; (2) the contents of the privacy policy are not too short. To be specific, 2KB is set as the lower bound size of the privacy policy documents; and (3) duplicated privacy policies, which are usually from different apps of the same company, are removed.
We crawl 1, 313 privacy policies and after filtering, 304 valid
privacy policies are left for annotation.



Store Listing

\cite{li2022understanding}

% \subsection{Status Quo of Data Safety Label in Google Play Store}
% Although Google required that every app needs to ...
% Market observations of datasets (similar to our APPG paper). E.g., How many apps failed to provide privacy labels? Which data type is the most collected? etc.

% How many missing?
% How many just provide a placeholder to meet the requirement?



% old google table
% \begin{table*}[htbp]
%   \caption{\faIcon{google} Performance of our proposed framework on the ground truth dataset. All the values are presented in percentages.}
%   \label{tab_google_results}
%   \vspace{-5pt}
%   \subfloat[Original ground truth dataset]{
%   \begin{tabular}{l r r r}
%     \toprule
%     \textbf{First-party collected} & \textbf{Precision} & \textbf{Recall} & \textbf{F1-score} \\
%     \midrule
%     \textbf{Data type} & 75.20 & 78.42 & 72.66\\

%     \textbf{Opt-in} & 66.56 & 75.05 & 62.49 \\
    
%     \textbf{Data type + Opt-in}  & 31.73 & 80.12 & 36.44\\


%     \midrule
%     \midrule
%         \textbf{Shared to third-party} & \textbf{Precision} & \textbf{Recall} & \textbf{F1-score} \\
%     \midrule
%     \textbf{Data type} & 66.80 & 75.26 & 63.15\\

%     \textbf{Opt-in} & 76.07 & 80.94 & 69.36 \\

%     \textbf{Data type + Opt-in}  & 34.08  & 64.21& 30.63\\
%     \midrule
%     \midrule
%         \textbf{Security practices} & \textbf{Precision} & \textbf{Recall} & \textbf{F1-score} \\
%     \midrule
%     \textbf{Encryption} & /  & / & 88.46\\
%     \textbf{RTBF} & /& / & 75.00 \\
%     \textbf{Encryption + RTBF} & 50.48& 90.38 & 51.98 \\
%   \bottomrule
% \end{tabular}
% }%
%  \quad 
%   \subfloat[Purified ground truth dataset (RQ1)]{
%   \begin{tabular}{l r r r}
%     \toprule
%     \textbf{First-party collected} & \textbf{Precision} & \textbf{Recall} & \textbf{F1-score} \\
%     \midrule
%     \textbf{Data type} & 67.50 & 74.86 & 62.94\\

%     \textbf{Opt-in} & 65.03 & 70.87 & 60.41 \\
    
%     \textbf{Data type + Opt-in}  & 38.22 & 78.32& 47.50\\
%     \midrule
%     \midrule
%         \textbf{Shared to third-party} & \textbf{Precision} & \textbf{Recall} & \textbf{F1-score} \\
%     \midrule
%     \textbf{Data type} & 63.68 & 75.63 & 60.00\\

%     \textbf{Opt-in} & 73.99 & 78.65 & 67.15 \\

%     \textbf{Data type + Opt-in}  &  35.62 & 70.71& 35.02\\
%     \midrule
%     \midrule
%         \textbf{Security practices} & \textbf{Precision} & \textbf{Recall} & \textbf{F1-score} \\
%     \midrule
%     \textbf{Encryption} & / & /& 89.64 \\
%     \textbf{RTBF} & / & / & 75.00 \\
%     \textbf{Encryption + RTBF} & 51.67 & 90.69 & 52.25 \\
%   \bottomrule
% \end{tabular}
% }%
% \end{table*}

==> Large_tables/apple_mapping.tex <==
\begin{table}[t!]
  \caption{\faIcon{apple} The mapping relations between high-level data practices mentioned in Section~\ref{sec_ContextClassificationModule}, and attributes in Apple's App Privacy Details. Category numbers without any mapping relation are omitted.}
  \label{tab_apple_mapping}
  \begin{tabular}{l c c }
    \toprule
    \textbf{Category No.} &1&2 \\
    \midrule
    \rowcolor{lightgray!85}
    Data linked to you &\checkmark&\\
    \rowcolor{lightgray!15}
    Data not linked to you &\checkmark& \\
    \rowcolor{lightgray!85}
    Data used to track you  &&\checkmark \\
\bottomrule
\end{tabular}
\end{table}

==> Large_tables/classifier_performance.tex <==
\begin{table}[htbp]
%   \caption{Classifier performance for high-level categories except \textit{`Other'} as implemented by Windl et al.~\cite{windl2022automating}.}
  \caption{The performance of the classification model that is used to predict the high-level categories of data practices.}
  \label{tab_classfier_performance}
  \resizebox{0.9\linewidth}{!}{%
  \begin{tabular}{l l c c c}
    \toprule
    \textbf{No.} &\textbf{Category} & \textbf{Prec.} & \textbf{Rec.} &  \textbf{F1-score}  \\
    \midrule
    1 &First-party Collection/Use & 0.87 & 0.75 & 0.80 \\
    2 &Third-party Sharing/Collection & 0.86 & 0.69 & 0.77 \\
    3 &User Access, Edit and Deletion & 0.73 & 0.65 & 0.69 \\
    4 &Data Retention & 0.54 & 0.31 & 0.39 \\
    5 &Data Security & 0.70 & 0.58 & 0.63 \\
    6&International \& Specific Audiences  & 0.96 & 0.84 & 0.90\\
    7 &Do Not Track & 1.00 & 1.00 & 1.00 \\
    8 &Policy Change & 0.86 & 0.67 & 0.75\\
    9 &User Choice/Control & 0.70 & 0.72 & 0.71 \\ 
    10 & Introductory/Generic &0.72 & 0.59 &0.65 \\
    11 & Practice not covered &0.59 &0.29 &0.39\\
    12 & Privacy contact information &0.84 &0.63 &0.72 \\
    \midrule
    \multicolumn{2}{l}{Average} & 0.79 & 0.65 & 0.70 \\

    
  \bottomrule
\end{tabular}
}%
\end{table}

==> Large_tables/google_mapping.tex <==
\begin{table}[t!]
  \caption{
%   \zc{\faIcon{google} ??what is this icon for?}\shidong{Help readers immediately recognise is the table/figures for Google or Apple dataset.} 
  \faIcon{google} The mapping relations between high-level data practices mentioned in Section~\ref{sec_ContextClassificationModule}, and attributes in Google's Data Safety Reports. Category numbers without any mapping relation are omitted. 
  \zc{1) Table heading is confusing. Rows are Data Safety Report Attributes in Table 2. Columns are data categories in Section 3.3. 2) You need to index data categories in Section 3.3 so that you can reference these categories by their indices here. 3) Table in between text is very strange.}}
  \label{tab_google_mapping}
  \begin{tabular}{l c c c c c c c c c}
    \toprule
    \textbf{Category No.} &1&2&3&4&5 \\
    \midrule
    \rowcolor{lightgray!85}
    First-party data collected &\checkmark&&&&\\
    \rowcolor{lightgray!15}
    Data shared to third-party &&\checkmark& &&\\
    \rowcolor{lightgray!85}
    Security practices - Encryption &&&&&\checkmark \\
    \rowcolor{lightgray!15}
    Security practices - RTBF &&&\checkmark&\checkmark& \\
\bottomrule
\end{tabular}
\end{table}
